SVEva Fair: A Framework for Evaluating Fairness in Speaker Verification

Despite the success of deep neural networks (DNNs) in enabling on-device voice assistants, increasing evidence of bias and discrimination in machine learning is raising the urgency of investigating the fairness of these systems. Speaker verification is a form of biometric identification that gives access to voice assistants. Due to a lack of fairness metrics and evaluation frameworks that are appropriate for testing the fairness of speaker verification components, little is known about how model performance varies across subgroups, and what factors influence performance variation. To tackle this emerging challenge, we design and develop SVEva Fair, an accessible, actionable and model-agnostic framework for evaluating the fairness of speaker verification components. The framework provides evaluation measures and visualisations to interrogate model performance across speaker subgroups and compare fairness between models. We demonstrate SVEva Fair in a case study with end-to-end DNNs trained on the VoxCeleb datasets to reveal potential bias in existing embedded speech recognition systems based on the demographic attributes of speakers. Our evaluation shows that publicly accessible benchmark models are not fair and consistently produce worse predictions for some nationalities, and for female speakers of most nationalities. To pave the way for fair and reliable embedded speaker verification, SVEva Fair has been implemented as an open-source python library and can be integrated into the embedded ML development pipeline to facilitate developers and researchers in troubleshooting unreliable speaker verification performance, and selecting high impact approaches for mitigating fairness challenges

==> notes/20210216_thoughts.tex <==
- Choose speaker verification and diarisation as scope
- Collect and review SOTA literature on speaker verification and diarisation (Google, Amazon, Facebook, Apple lead researchers)
    Alexander Gruenstein
    Ian McGraw
    
- Review fairness metrics
- Make a table of SOTA models [non-compressed and compressed] | framework | model url | code url
- Make a table of common compression approaches and their implementations

Core question: does fairness of speaker verification and diarisation models deteriorate for compressed models?

==> notes/archive.tex <==
\subsection{Evaluating Fairness of ML-based systems}
highlight new angle - speaker verification and fairness
\cite{Martinez2021Software} - software engineering for AI-based systems
Testing approaches
Structural coverage (neuron-based perspective), non-structural coverage
\cite{Sun2018Testing} Testing Deep Neural Networks \cite{Balkan2017Underminer}
\cite{Asyrofi2020Crossasr}
\cite{Aggarwal2019Black} Black box fairness testing of machine learning models:  ML only, not suitable for deep learning and embedded ML
\cite{Saleiro2018Aequitas} AEQUITAS, a bias and fairness audit toolkit to detect discrimination and bias for predictive risk assessment 
\cite{Bellamy2019Ai} AI fairness 360 - corporate; allocation or risk assessment problems with well-defined protected attributes in which one would like to have some sort of statistical or mathematical notion of sameness
TensorFlow Fairness Indicator (no speaker verification)

General testing ML systems
MLPerf
\cite{Riccio2020Testing}
